Analytic Manifold Learning: Unifying and Evaluating Representations for Continuous Control

We address the problem of learning reusable state representations from streaming high-dimensional observations. This is important for areas like Reinforcement Learning (RL), which yields non-stationary data distributions during training. We make two key contributions. First, we propose an evaluation suite that measures alignment between latent and true low-dimensional states. We benchmark several widely used unsupervised learning approaches. This uncovers the strengths and limitations of existing approaches that impose additional constraints/objectives on the latent space. Our second contribution is a unifying mathematical formulation for learning latent relations. We learn analytic relations on source domains, then use these relations to help structure the latent space when learning on target domains. This formulation enables a more general, flexible and principled way of shaping the latent space. It formalizes the notion of learning independent relations, without imposing restrictive simplifying assumptions or requiring domain-specific information. We present mathematical properties, concrete algorithms for implementation and experimental validation of successful learning and transfer of latent relations.

==> approach_experiments_old.tex <==
%=================================================
\section{Evaluating {\ouralgofullname}  ({\ouralgo})}

\begin{figure}[t]
\centering
\includegraphics[width=1\textwidth]{img/aml_train/AnalyticFullDomainAndSyz}
\includegraphics[width=1\textwidth]{img/aml_train/AnalyticFullTransverse}
\vspace{-15px}
\caption{Learning relations $g_1,..,g_k$ on a noisy version of the analytic domain.}
\label{fig:amlanalytic}
\vspace{-5px}
\end{figure}

We evaluate our {\ouralgo} approach with 3 sets of experiments: 1) learning on an analytic domain and visualizing relations in 3D; 2) handling dynamics with friction and drag on a \textit{block-on-incline} domain; 3) employing learned relations to get improved representations on the \textit{YCB-on-incline} target domain.

For our analytic domain on-manifold data comes from an intersection of a hyperboloid and a plane. The top row of Figure~\ref{fig:amlanalytic} shows results using restricted syzygies. We visualize $g_1 \cap g_2 \cap ... \cap g_5$: the intersection of the learned relations $g_1,...,g_5$ (i.e. the intersection of the zero-level sets of these relations). The \mbox{zero-level} sets of individual relations are shown next.
On the second row, we show training with transversality: $g_1 \cap g_2$ has two simple relations -- a plane and a hollow cylinder; $g_1 \cap g_2 \cap g_3 \cap g_4$ includes smoothed cones. Transversality allows capturing information with a small number of general relations. In contrast, relations found using syzygies have more complicated shapes and can be similar in some regions, as expected. This could be useful when we need to avoid large changes, e.g. for fine-tuning or for flexible partial transfer using subsets of relations.

\begin{figure}[b]
\centering
\vspace{-15px}
\includegraphics[width=0.188\textwidth]{img/aml_train/AML_BlockOnIncline45Tn_transverse_200531_120903_onmanifold_wider}
\hspace{-4px}
\includegraphics[width=0.15\textwidth]{img/aml_train/AML_BlockOnIncline45Tn_transverse_200531_120903_intersection}
\includegraphics[width=0.166\textwidth]{img/aml_train/AML_BlockOnIncline35TnFric_transverse_200531_144704_onmanifold_tight}
\includegraphics[width=0.15\textwidth]{img/aml_train/AML_BlockOnIncline35TnFric_transverse_200531_144704_intersection}
\includegraphics[width=0.166\textwidth]{img/aml_train/AML_BlockOnInclineTnDrag_transverse_200531_120916_onmanifold_tight}
\includegraphics[width=0.15\textwidth]{img/aml_train/AML_BlockOnInclineTnDrag_transverse_200531_120916_intersection}
\vspace{-15px}
\caption{Phase space plots for on-manifold data and relations learned with {\ouralgo} for \textit{block-on-incline}. 
}
\label{fig:amlblock}
\vspace{-1px}
\end{figure}
Next, we evaluate {\ouralgo} on a physics domain: a block sliding down an incline. 
The block is given a random initial velocity; gravity, friction and drag forces then determine its further motion. On-manifold data consists of noisy position \& velocity of the block at the start and end of trajectories.
Figure~\ref{fig:amlblock} shows {\ouralgo} with transversality (Appendix~\ref{sec:suppl_b33} gives results with syzygies). We visualize phase space plots: arrows show change in position \& velocity after $1sec$ of sliding (scaled to fit). The left plots show the case of a $45^{\circ}$ incline and demonstrate generalization. {\ouralgo} is only given training data with start position \& velocity $\in [0,0.2]$, but is able to generalize to $[0,0.4]$.
The middle plots show high friction on a $35^{\circ}$ incline. The right plots show high drag on a $10^{\circ}$ incline. 
Overall, these results show that {\ouralgo} can generalize beyond training data ranges and capture non-linear dynamics.

Lastly, we show transfer to \textit{YCB-on-incline} domain (rightmost in Figure~\ref{fig:envs}) and compare AML to the leading approaches from our earlier experiments: $P\!RED$ and $V\!\!AE_{rpl}$. We note that while $SP\!AIR$ did ok on \textit{RearrangeGeom}, it had significant problems reconstructing existing benchmarks. Decoding \textit{RearrangeYCB} was problematic for all approaches (see Appendix~\ref{sec:suppl_a}). Even supervised decoder training failed (with true states as training input). Decoder design is outside the scope of this work. Hence, we evaluate {\ouralgo} transfer using \textit{YCB-on-incline}, which has challenging dynamics \& images, but is still tractable for decoding.
%
First, {\ouralgo} learns relations from \textit{Geom-on-incline}. Incline angle, friction and object pose are initialized randomly.
Actions are random forces that push objects along the incline. {\ouralgo} is given incline, position \& velocity at two subsequent steps, and the applied action.

\begin{wrapfigure}{r}{0.29\textwidth}
\centering
\vspace{-12px}
\includegraphics[width=0.29\textwidth]{img/aml_rl/aml_ycb_incline_ld_pos_err_rand}
\includegraphics[width=0.29\textwidth]{img/aml_rl/aml_ycb_incline_ld_distortion_variability}
\vspace{-14px}
\caption{\textit{YCB-on-incline}: mean of 6 training runs, shaded areas show one STD.}
\label{fig:sliding_ycb_aml}
\vspace{-40px}
\end{wrapfigure}
Then, we train an unsupervised learner ($P\!RED$) on the target \textit{YCB-on-incline} domain. PPO RL drives the distribution of RGB frames. RL gets high rewards for pushing objects to stay in the middle of the incline.
%
We impose {\ouralgo} relations by extending the latent part of an ELBO-based loss (with $z_{t,\tnxt}$ as encoder outputs):
$
\mathcal{L} \!=\! -\!\big[\underbrace{\log p(x|z_{t,\tnxt}\!) \!\!-\!\! K\!L\big(q(\!z_{t,\tnxt}\!)|\!|\mathcal{N}\!(0,\!1\!)\big)}_{\text{standard } ELBO \text{ for } P\!RED \text{ version of } V\!AE}\big] \!+\! \underbrace{\textstyle\sum_{k=1}^K \big|g_k(\!z_{t,\tnxt},\!a_t\!)\big|}_{\text{impose } {\ouralgo} \text{ relations}}
$
The resulting {\ouralgo}$_{\text{trnsv}}$ ({\ouralgo}$_{\text{syz}}$ when using syzygies) gets a better latent state alignment for object position compared to $V\!\!AE_{rpl}$ and $P\!RED$ without {\ouralgo} relations imposed (see the top plot in Figure~\ref{fig:sliding_ycb_aml}).

Another important quality measure of a latent space mapping is how much it distorts the true data manifold. We quantify this as follows (on 10K test points): take pairs of low-dimensional representations $\tau_1^{true}$, $\tau_2^{true}$ and the corresponding pixel-based representations $x_1, x_2$, then compute distortion coefficient $\rho_{distort} \!=\! \log \big[ d_{L2}\big(\phi_{enc}(x_1), \phi_{enc}(x_2)\big) \big/ d_{L2}\big(\tau_1^{true}, \tau_2^{true}\big) \big]$,
with $d_{L2}$ as Euclidean distance. An encoder that yields low variance of these coefficients better preserves the geometry of the low-dimensional manifold (up to overall scale). This measure is related to approaches surveyed in~\cite{distort18, bartal2019dimensionality} (see Appendix~\ref{sec:suppl_b32}).
The bottom plot in Figure~\ref{fig:sliding_ycb_aml} confirms that {\ouralgo} helps achieving lower distortion variability.

Results presented in Figure~\ref{fig:sliding_ycb_aml} show that imposing {\ouralgo} relations helps improve the latent space mapping of $P\!RED$ when training on RGB frames. The distribution of the frames is non-stationary, since they are sampled using the current (changing) policy of an RL learner.
Overall, this above setup aims to demonstrate the potential for sim-to-real transfer. In this case, \textit{Geom-on-incline} plays a role of a simulator, while frames from \textit{YCB-on-incline} act as surrogates for `real' observations. Note that YCB objects have realistic visual appearances and their dynamics is dictated by meshes obtained from the 3D scans of real objects. Hence, there is a non-trivial mismatch between the dynamics of the simple shapes of \textit{Geom-on-incline} domain vs realistic shapes of the \textit{YCB-on-incline} domain.

